Computational Complexity of Hedonic Games on Sparse Graphs

The additively separable hedonic game (ASHG) is a model of coalition formation games on graphs. In this paper, we intensively and extensively investigate the computational complexity of finding several desirable solutions, such as a Nash stable solution, a maximum utilitarian solution, and a maximum egalitarian solution in ASHGs on sparse graphs including bounded-degree graphs, bounded-treewidth graphs, and near-planar graphs. For example, we show that finding a maximum egalitarian solution is weakly NP-hard even on graphs of treewidth 2, whereas it can be solvable in polynomial time on trees. Moreover, we give a pseudo fixed parameter algorithm when parameterized by treewidth.

==> asymmetric.tex <==
%\section{Asymmetric Variant}\label{sec:asymmetric}

%In this section, we consider asymmetric variants of hedonic games.
%We can observe that Theorems~\ref{thm:treewidth:hedonic} and \ref{thm:pseudo_tw:Egal} hold for asymmetric hedonic games.


==> k-forming.tex <==
\section{Max Utilitarian Partition}

\begin{theorem}\label{thm:tw^tw}
Given a tree decomposition of width $\tw$, \textsc{Max Utilitarian Partition} can be solved in time $O((\tw+1)^{\tw+1}(\tw+k)kn)$.
\end{theorem}
\begin{proof}
Our algorithm is based on standard dynamic programming on a tree decomposition.
In our dynamic programming, we keep track of all the partitions in each bags.



We define recursive formulas for computing the social welfare of each partition ${\mathcal P}_i$ in the subgraph based on a subtree of a tree decomposition. 
We denote by $A^{(p)}_i[{\mathcal P}_i]$ of  the maximum social welfare for ${\mathcal P_i}$ such that the number of coalitions until node $i$ is $p$. 
Notice that $A^{(k)}_r[\emptyset]$ in root node $r$ is the maximum social welfare of $G$.
We denote a parent node by $i$ and its child node by $j$. For a join node, we write $j_1$ and $j_2$ to denote its two children. 

\paragraph*{Leaf node:}  
In leaf nodes, we set $A^{(0)}_i[\emptyset]=0$ if $p=0$ and otherwise $A^{(p)}_i[\emptyset]=-\infty$ if $p\in \{1,\ldots, k\}$. 


\paragraph*{Introduce vertex $v$ node:} 
In an introduce vertex $v$ node $i$, let $C_v\in {\mathcal P}_i$ be the coalition including $v$ and  ${\mathcal P}_j = {\mathcal P}_i \setminus \{C_v\} \cup \{C_v\setminus \{v\}\}$. We notice that the social welfare is changed only in the coalition including $v$. 
For $p\ge 1$, the recursive formula is defined as: 
\[
 A^{(p)}_i[{\mathcal P}_i]=\begin{cases} 
A^{(p)}_j[{\mathcal P}_j]+\sum_{(u,v)\in G[C_v]} w_{uv} & \mbox{if $C_v\neq \{v\}$}\\
A^{(p-1)}_j[{\mathcal P}_j] &\mbox{otherwise}.
\end{cases}
\]
In the former case, $v$ is contained in an existing coalition.
On the other hand, $v$ creates a new coalition containing only itself in the latter case. 
For $p=0$, we set  $A^{(p)}_i[{\mathcal P}_i]=-\infty$ because if there is a vertex in a bag, the number of coalition is at least one.


\paragraph*{Forget $v$ node:}
In a forget $v$ node, we only take a partition with maximum social welfare when we forget $v$ because $v$ does not affect the social welfare hereinafter.
Furthermore, the number of coalitions does not change.
Thus, the recursive formula is defined as: 
$$A^{(p)}_i[{\mathcal P}_i]=\max_{{\mathcal P}_j\in {\mathcal D}_j} A^{(p)}_j[{\mathcal P}_j]$$ 
where ${\mathcal D}_j=\{{\mathcal P}_j \mid {\mathcal P}_j \setminus \{C_v\} \cup \{C_v\setminus \{v\}\}={\mathcal P}_i\}$.
Note that the size of ${\mathcal D}_j$ is at most $\tw+1$.

\paragraph*{Join node:}
A join node $i$ has two child nodes $j_1, j_2$ where $X_i=X_{j_1}=X_{j_2}$.
The social welfare of each partition $X_i$ is the sum of the corresponding partition of $X_{j_1}=X_{j_2}$.
Let $p_{j_1}$ and $p_{j_2}$ be  the number of coalitions until node $j_1$ and $j_2$, respectively.
Then, the number of coalitions $p$ in node $i$ is $p_{j_1}+p_{j_2}-|{\mathcal P}_i|$.
Therefore,  the recursive formula for a join node is defined as:
$$A^{(p)}_i[{\mathcal P}_i]=\max_{p_{j_1}+p_{j_2}-|{\mathcal P}_i|=p} \{A^{(p_{j_1})}_{j_1}[{\mathcal P}_{i}]+A^{(p_{j_2})}_{j_2}[{\mathcal P}_{i}]\}.$$ 
Notice that $|{\mathcal P}_i|+p$ is at most $\tw+k+2$.

The running time of each row of $A^{(p)}_i[{\mathcal P}_i]$ for an introduce node, a forget node, and a join node is $\tw+1$, $\tw+1$, $\tw+k+2$, respectively.
Because the size of each DP table is $O((\tw+1)^{\tw+1}k)$, we can compute the recursive formulas for each node in time $O((\tw+1)^{\tw+1}k(\tw+k+2))$.
As the result, we have the total running time $O((\tw+1)^{\tw+1}(\tw+k)kn)$.
\end{proof}
Since $k\le n$, \textsc{Max Utilitarian Partition} is FPT parameterized by treewidth.


If we replace  $A^{(p)}_i[{\mathcal P}_i]=A^{(p)}_j[{\mathcal P}_j]+\sum_{(u,v)\in G[C_v]} w_{uv}$ by $A^{(p)}_i[{\mathcal P}_i]=A^{(p)}_j[{\mathcal P}_j]+\prod_{(u,v)\in G[C_v]} w_{uv}$ in an introduce node, we can compute Nash Social Welfare Maximization in the same time.
\begin{corollary}
Given a tree decomposition of width $\tw$, \textsc{Max Nash Utilitarian Partition} can be solved in time $O((\tw+1)^{\tw+1}(\tw+k)kn)$.
\end{corollary}

\begin{corollary}
Given a tree decomposition of width $\tw$, \textsc{Max $k$-Cut} can be computed in time $O((\tw+1)^{\tw+1}(\tw+k)kn)$.
\end{corollary}

On the other hand, \textsc{Max Egalitarian Partition} is paraNP-hard parameterized by vertex cover.
\begin{theorem}
\textsc{Max Egalitarian Partition} is NP-hard on graphs of vertex cover number two even if the preferences are nonnegative.
\end{theorem}
\begin{proof}
Reduction from \textsc{Partition}.
\end{proof}

\paragraph*{Note}
\begin{itemize}
\item $k$-formingはpreference $f$をsymmetricと最初から仮定している．すなわち，$f_u(v)=f_v(u)$ for $(u,v)\in E$としている．ただし，\textsc{Max Utilitarian Partition}と\textsc{Max Nash Utilitarian Partition}は，それぞれ辺重みを$w_{uv}=f_u(v)+f_v(u)$, $w_{uv}=f_u(v)\cdot f_v(u)$とすれば動く．


 
\item また，\textsc{Max Utilitarian Partition}が常にgroup stableになるのは，symmetricが強く効いているので(たぶんpotential functionの議論)，asymmetricでどうか考える必要あり．hedonic gameの証明をなぞればいける？

\item 安定解の定義をきちんとする必要あり．
\item Nash-安定解の存在判定はNP-cの証明を読むと、Exact 3 coverからの帰着ということもあり、k=n/3の時、k-formingの安定解存在判定はNP-cであることがわかります。(と思ったのですが、k-formingにおける安定解をどう定義するかに依ります) ただ、完全グラフにおいてであり、スパースなグラフではわかりません。

\item kがfixされているときはどうなのかはやる価値あるかなと。特にk=2,3のとき。
Coreの存在性判定は、kが3以上でNP-c(theorem 7)ですが、k=2はどうなのか書いてあるかみる必要あります。
\item Exchanging stability?

\item assymmetricで，正重みしかないときに，stable解，core解が常に存在するのか，するならPoS, PoA, 存在しないなら存在性判定の計算困難性を調べるのは通常のhedonic gameでは考えられない事柄です．

\item 木とかのスパースなグラフで色々やって、実際の社会ネットワークはスパースであるからやったというストーリーで書けばちょっと有用性があるように見えるかもです。
 \end{itemize}
